Exotic Newton-Hooke group, noncommutative plane and superconformal symmetry

In this thesis some systems with exotic symmetries, which are a peculiarity in 2+1 space-time dimensions, are studied. Coded in the exotic structure, there appear noncommutative coordinates and a phases structure. This kind of systems has attracted attention from different areas of physics independently. Among them, we can mention: theory of ray representations of Lie groups, anyon physics, some condensed matter systems, for instance the quantum Hall effect, planar gauge and gravitation theories, noncommutative field theory, noncommutative geometry, and noncommutative quantum mechanics. We focus our study in some topics on exotic nonrelativistic symmetries, such as the exotic Newton-Hooke group, the relation between such systems and the noncommutative Landau problem, the symmetries of noncommutative Landau problem, and of its supersymmetric extension. The exotic Newton-Hooke group corresponds to the nonrelativistic limit of the de Sitter groups, and has as a particular, flat limit the exotic Galilei group. For the exotic Newton-Hooke symmetry, we construct a free particle action, and realize a complete study of its classical and quantum properties. The Newton-Hooke system is intimately related with the noncommutative Landau problem, which we study apart. We show that the inclusion of spin degrees of freedom in the noncommutative Landau problem produces a natural integration of the exotic Newton-Hooke group with the conformal symmetry and supersymmetry.

==> def.tex <==
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%inicios de capitulos mas bonitos...%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\@makechapterhead#1{%
%  \vspace*{20\p@}%
%  {\parindent \z@ \raggedright
%    \normalfont
%    \ifnum \c@secnumdepth >\m@ne
%      \if@mainmatter
%        %\huge\bfseries
%        \scshape
%        \@chapapp\space \thechapter
%        \par\nobreak
%%        \vskip 20\p@
%      \fi
%    \fi
%    \interlinepenalty\@M
%    \Huge \bfseries #1\par\nobreak
%    \vskip 40\p@
%  }}
%\def\@schapter#1{\if@twocolumn
%                   \@topnewpage[\@makeschapterhead{#1}]%
%                 \else
%                   \@makeschapterhead{#1}%
%                   \@afterheading
%                 \fi}
%\def\@makeschapterhead#1{%
%  \vspace*{20\p@}%
%  {\parindent \z@ \raggedright
%    \normalfont
%    \scshape
%    \interlinepenalty\@M
%    \Huge \bfseries #1\par\nobreak
%    \vskip 40\p@
%  }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%comandos nuevos...%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\half}{{\scriptstyle{\frac{1}{2}}}}
\def\vb{{\vec b}}
\def\vc{{\vec c}}

\def\nn{\nonumber}
\def\z{\zeta}
\newcommand{\T}{\theta}

\newcommand{\W}{\Omega}
\def\Z{\mathbb Z}
\newcommand{\h}{\eta}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\def\d{\dot}

\def\nn{\nonumber}
\newcommand{\bref}[1]{(\ref{#1})}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%cambio de nombres de objetos...%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\renewcommand{\contentsname}{Índice general}
%\renewcommand{\bibname}{Bibliografía}
%\renewcommand{\tablename}{Tabla}
%\renewcommand{\figurename}{Figura}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%indice mas bonito...%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%nuevos margenes de pagina...%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\linespread{1.2}
\textwidth16.8cm
\textheight23cm
\setlength{\headheight} {18pt}

%%%para ambas caras de impresion...%%%%%%%%%%%%%%%%%%%%%%
\setlength{\oddsidemargin}  {0.5cm}
\setlength{\evensidemargin}{-1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%una sola cara de impresion...%%%%%%%%%%%%%%%%%%%%%%%%%
%\setlength{\oddsidemargin}  {0.5cm}
%\setlength{\evensidemargin}  {0.5cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\marginparwidth} {76pt}
\hoffset=0cm
\headsep=1cm
\voffset=-2.0cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%fancy pages - una cara de impresion (new tops)...%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\makeindex
%\urlstyle{rm}
%\fancyhead{}
%  \fancyhead[LO,LE]{\slshape \rightmark}
%  \fancyhead[RO,RE]{\thepage}
%%  \fancyhead[RE]{\slshape \leftmark}
%  \fancyfoot{}
%  \pagestyle{fancy}
%  \renewcommand{\chaptermark}[1]{\markboth{\chaptername \ \thechapter \ \ #1}{}}
%  \renewcommand{\sectionmark}[1]{\markright{\thesection \ \ #1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%fancy pages - ambas caras de impresion (new tops)...%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\makeindex
%\urlstyle{rm}
%\fancyhead{}
%  \fancyhead[LO]{\slshape \rightmark}
%  \fancyhead[RO,LE]{\thepage}
%  \fancyhead[RE]{\slshape \leftmark}
%  \fancyfoot{}
%  \pagestyle{fancy}
%  \renewcommand{\chaptermark}[1]{\markboth{\chaptername \ \thechapter \ \ #1}{}}
%  \renewcommand{\sectionmark}[1]{\markright{\thesection \ \ #1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






